Diversity-Driven Exploration Strategy for Deep Reinforcement Learning

Efficient exploration remains a challenging research problem in reinforcement learning, especially when an environment contains large state spaces, deceptive local optima, or sparse rewards. To tackle this problem, we present a diversity-driven approach for exploration, which can be easily combined with both off- and on-policy reinforcement learning algorithms. We show that by simply adding a distance measure to the loss function, the proposed methodology significantly enhances an agent's exploratory behaviors, and thus preventing the policy from being trapped in local optima. We further propose an adaptive scaling method for stabilizing the learning process. Our experimental results in Atari 2600 show that our method outperforms baseline approaches in several tasks in terms of mean scores and exploration efficiency.

==> deprecated/custom_packages.tex <==
% AMS mathematical facilities for LATEX
\usepackage{amsmath}
% Customising captions in floating environments
\usepackage[font=small]{caption}
% Control layout of itemize, enumerate, description
\usepackage{enumitem}
% Mathematical tools to use with amsmath
\usepackage{mathtools}
% Select alternative section titles
\usepackage{titlesec}

% Kills all vertical spacing in items and between items and paragraphs
\setlist{nosep}

% Change spacing around the title
\titlespacing{\chapter}{0pt}{*.1}{*.1}
\titlespacing{\section}{0pt}{*.1}{*.1}
\titlespacing{\subsection}{0pt}{*.1}{*.1}
\titlespacing{\subsubsection}{0pt}{*.1}{*.1}
\titlespacing{\paragraph}{0pt}{*.1}{*1}
\titlespacing{\subparagraph}{0pt}{*.1}{*1}

% Change spacing after tables
\captionsetup[table]{skip=1ex}

% Change spacing around captions
\setlength{\belowcaptionskip}{-3ex}

% Bibliography style
\bibliographystyle{unsrtnat}

% Math operators
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% Remove the ugly borders around references and hyperlinks
% Tricks to make all links and citations look good
\hypersetup{%
    pdfborder = {0 0 0},
    colorlinks = true, %Colored links instead of ugly boxes
    urlcolor = blue, %Color for external hyperlinks
    linkcolor = blue, %Color of internal links
    citecolor = red %Color of citations
}
